Typed Decision Models under Prevalence Shift and Label Budgets: Decision Training, Calibration, and Implicit Priors

Typed decision models (TDMs) return probabilities over caller-defined options, and Jev's vendor describes it as calibrated. We ask whether vendor decision training improves a model over its backbone, whether a TDM's calibration and thresholds withstand prevalence (label) shift like a fine-tuned classifier's, and how many labels a trained model needs to overtake a TDM. We compare three TDMs (Jev, Tev1-4B, Nimble-9B), their base models and trained classifiers on identical candidate-set decisions from five public datasets (on intent datasets, within the gold label's intent group) under simulated shift, with 35 paired tests frozen before the confirmatory analysis (earlier test-data checks disclosed), and estimate label-budget curves. First, decision training is not always beneficial: Nimble-9B, which differs from Qwen3.5-9B only by a LoRA adapter, is better calibrated on intent tasks but 12 Macro-F1 points worse on financial sentiment, a loss that persists across prompt formats; Tev1-4B's largest gain over its backbone is a prompt-format effect. Second, on 50 fixed moderate shifts, Jev's top-label calibration error and threshold risk grow significantly more than a fine-tuned DeBERTa's only on financial sentiment, sensitive to the prior set; averaged over 2,000 shifts the gap is at most one point. Third, label-free EM correction with the model's implicit prior lowers Jev's shifted calibration error where it is highest, but labelled recalibration lowers it far more. Fourth, DeBERTa needs 100-250 labels to overtake Jev on hate speech and does not clearly overtake it on CLINC150 at any budget; a QLoRA adapter on Qwen3.5-4B overtakes Jev with at most 2,500 labels on every dataset, on CLINC150 only marginally and not under in-budget selection. The TDMs tested are neither uniformly better than their backbones nor uniquely fragile under shift; their lead over trained models depends on the task.

==> tables/tab_calib_robust_pairs.tex <==
\begin{tabular}{llrrrrr}
\toprule
Comparison & Metric & CLINC150 & HWU64 & FPB & HateXplain & TREC-6 \\
\midrule
Tev1-4B $-$ Qwen3.5-4B & Top-label ECE, equal width (paper) & $-$0.3 & $-$1.9 & $-$13.2 & $-$3.2 & +0.1 \\
 & Top-label ECE, equal mass & $-$0.5 & $-$1.7 & $-$11.9 & $-$3.2 & +1.1 \\
 & Debiased calibration error & $-$1.4 & $-$2.9 & $-$12.5 & $-$4.2 & +2.4 \\
 & Class-wise ECE & $-$0.3 & $-$0.2 & $-$9.4 & $-$2.3 & +0.9 \\
 & Brier score & $-$3.4 & $-$4.7 & $-$20.7 & $-$3.8 & +1.2 \\
\midrule
Nimble-9B $-$ Qwen3.5-9B & Top-label ECE, equal width (paper) & $-$1.2 & $-$4.2 & +9.6 & $-$0.4 & $-$1.8 \\
 & Top-label ECE, equal mass & $-$1.2 & $-$4.6 & +9.5 & $-$0.4 & $-$1.9 \\
 & Debiased calibration error & $-$2.9 & $-$8.9 & +12.4 & $-$0.7 & $-$6.9 \\
 & Class-wise ECE & 0.0 & $-$0.1 & +10.8 & +0.3 & +1.0 \\
 & Brier score & $-$0.7 & $-$3.5 & +20.9 & $-$0.2 & +3.3 \\
\midrule
Jev $-$ DeBERTa-v3-large & Top-label ECE, equal width (paper) & $-$0.5 & +0.6 & $-$1.6 & +13.8 & +2.1 \\
 & Top-label ECE, equal mass & $-$0.7 & +1.1 & $-$1.2 & +14.0 & +0.9 \\
 & Debiased calibration error & $-$2.2 & +1.0 & $-$2.8 & +14.2 & $-$1.0 \\
 & Class-wise ECE & +0.1 & +0.3 & +4.0 & +11.8 & +1.5 \\
 & Brier score & +0.2 & +4.4 & +13.8 & +27.1 & +7.5 \\
\bottomrule
\end{tabular}


==> tables/tab_calib_robust_shift.tex <==
\begin{tabular}{lrrrrr}
\toprule
Metric & CLINC150 & HWU64 & FPB & HateXplain & TREC-6 \\
\midrule
Top-label ECE, equal width (paper) & 0.0 & +0.1 & +0.2 & $-$0.8 & +1.0 \\
Top-label ECE, equal mass & 0.0 & 0.0 & +0.3 & $-$0.9 & +1.0 \\
Debiased calibration error & +0.3 & +0.1 & $-$1.0 & $-$1.1 & +3.0 \\
Class-wise ECE & 0.0 & 0.0 & +1.8 & $-$1.4 & +0.3 \\
Brier score & 0.0 & $-$0.1 & +0.2 & $-$1.6 & +1.0 \\
\bottomrule
\end{tabular}


==> tables/tab_pa_seed_bootstrap.tex <==
\begin{tabular}{llrrrrr}
\toprule
Test & Bootstrap & CLINC150 & HWU64 & FPB & HateXplain & TREC-6 \\
\midrule
PA1 & seed 1001 (frozen) & +0.1 [$-$0.0, +0.2] & +0.1 [$-$0.3, +0.5] & +1.7 [+1.0, +2.5] & $-$0.8 [$-$1.3, $-$0.3] & +1.0 [+0.3, +1.8] \\
 & seeds resampled & +0.1 [$-$0.0, +0.2] & +0.2 [$-$0.2, +0.6] & +1.5 [+0.7, +2.3] & $-$1.3 [$-$3.4, $-$0.3] & +1.0 [+0.2, +1.8] \\
\midrule
PA2 & seed 1001 (frozen) & $-$0.0 [$-$0.0, +0.0] & +0.0 [$-$0.2, +0.2] & +2.5 [+1.8, +3.2] & $-$0.6 [$-$1.0, $-$0.1] & +0.5 [$-$0.1, +1.3] \\
 & seeds resampled & $-$0.0 [$-$0.0, +0.0] & $-$0.0 [$-$0.2, +0.2] & +2.4 [+1.5, +3.4] & $-$0.6 [$-$1.1, $-$0.2] & +0.5 [$-$0.2, +1.3] \\
\bottomrule
\end{tabular}


==> tables/tab_router.tex <==
\begin{tabular}{lrrrr}
\toprule
 & \multicolumn{2}{c}{CLINC150} & \multicolumn{2}{c}{HWU64} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
Accuracy & gold group & routed & gold group & routed \\
\midrule
Router (group accuracy) & -- & 0.938 & -- & 0.930 \\
\midrule
Jev & 0.978 & 0.918 & 0.911 & 0.850 \\
Tev1-4B & 0.964 & 0.905 & 0.891 & 0.832 \\
Nimble-9B & 0.962 & 0.904 & 0.897 & 0.836 \\
Qwen3.5-4B & 0.939 & 0.884 & 0.862 & 0.801 \\
Qwen3.5-9B & 0.955 & 0.898 & 0.880 & 0.821 \\
DeBERTa-v3-large & 0.980 & 0.923 & 0.943 & 0.882 \\
TF-IDF + LR & 0.950 & 0.899 & 0.901 & 0.849 \\
\bottomrule
\end{tabular}

